FLAMES: Improving LLM Math Reasoning via a Fine-Grained Analysis of the Data Synthesis Pipeline

Recent works improving LLM math reasoning with synthetic data have used unique setups, making comparison of data synthesis strategies impractical. This leaves many unanswered questions about the roles of different factors in the synthetic data pipeline, such as the impact of filtering low-quality problems. To address this gap, we introduce FLAMES, a Framework for LLM Assessment of Math rEasoning Data Synthesis, and perform a systematic study of 10 existing data synthesis strategies and multiple other factors impacting the performance of synthetic math reasoning data. Our FLAMES experiments provide several valuable insights about the optimal balance of difficulty and diversity of synthetic data. First, data agents designed to increase problem complexity lead to best improvements on most math metrics. Second, with a fixed data generation budget, keeping higher problem coverage is more important than keeping only problems with reliable solutions. Third, GSM8K- and MATH-based synthetic data can lead to improvements on competition-level benchmarks, showcasing easy-to-hard generalization. Leveraging insights from our FLAMES experiments, we design two novel data synthesis strategies for improving out-of-domain generalization and robustness. Further, we develop the FLAMES dataset, an effective blend of our novel and existing data synthesis strategies, outperforming public datasets on OlympiadBench (+15.7), CollegeMath (+4.5), GSMPlus (+6.5), and MATH (+3.1). Fine-tuning Qwen2.5-Math-7B on the FLAMES dataset achieves 81.4% on MATH, surpassing larger Llama3 405B, GPT-4o and Claude 3.5 Sonnet.

==> sections/01_Introduction.tex <==
\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figures/model_comparisonv2.png}
  %\caption{Results of different LLMs on the MATH benchmark. Fine-tuning Qwen2.5-Math-7B with our FLAMES\_large dataset improves performance more than any open-source math dataset (e.g. OrcaMath), and over several open-source and proprietary models}
  \caption{MATH benchmark score for popular LLMs. Qwen2.5-Math-7B + X (FLAMES or OrcaMath) denotes results obtained by finetuning Qwen2.5-Math-7B model with X dataset. Comparison of FLAMES data with other public Math datasets is shown in Table \ref{tab:open-source}.}
  \label{fig:experiments}
\end{figure}

\section{Introduction}
% \vspace{-5}

\begin{figure}[t]
 % \centering
  \includegraphics[width=\columnwidth]{figures/preview_draftv2.png}
  % \includegraphics[width=2.0\columnwidth]{figures/preview_draftv2.png}
  \caption{The landscape of recently-proposed synthetic math reasoning strategies. Each work uses different synthesis models, student models, and quality control methods, making comparison of problem synthesis agents impractical.}
  \label{fig:preview}
\end{figure}

%  Agentic Framework for Optimized EXploration of Math Reasoning Data Synthesis (Agentic FOX framework)

% FLAMES: \underline{F}ramework for \underline{L}LM \underline{A}ssessment of \underline{M}ath r\underline{E}asoning with Data \underline{S}ynthesis

Solving math problems has been a key measure of evaluating the reasoning ability of large language models (LLMs) \ignore{in the field of natural language processing (NLP)} \cite{wei2022chain, cobbe2021training, hendrycks2measuring}. Due to the challenges of creating a large-scale human-crafted dataset, LLM-based generation of synthetic data has been explored and proven effective in improving LLM math reasoning capabilities \cite{metamath, kpdds, scalequest}. While early works on math reasoning data synthesis focused on synthesis of solutions for existing problems, e.g. rejection sampling \cite{Tong2024DARTMathDR}, recent works have shifted focus towards increasing problem diversity by synthesizing new problems. Recent works such as Orca-Math \cite{orcamath}, MetaMath \cite{metamath}, and OpenMath-Instruct-2 \cite{omi2} have proposed one or more strategies\footnote{These data synthesis strategies often use one or multiple LLM calls and are commonly referred to as data generating agents, or data agents. We use the terms \textit{strategies} and \textit{agents} interchangeably in this paper.} for generating new math problems. However, these works use non-standard setups, making the comparison of data synthesis strategies across studies infeasible. This lack of standardization deprives researchers and practitioners of practical insights, leaving them uninformed about the real factors driving performance improvements via math reasoning data synthesis. 


Figure \ref{fig:preview} highlights the lack of standardization by summarizing setups of four popular math reasoning data synthesis works in terms of four experimental design decisions. As evident in Figure \ref{fig:preview}, it is infeasible to conclude whether Suggester-Editor \cite{orcamath} is a better data synthesis strategy or question fine-tuning (QFT) \cite{scalequest}, as different problem synthesis models and student models have been used in the OrcaMath and ScaleQuest papers. 

This lack of standardization poses several previously-under-studied research questions about math reasoning data synthesis. \underline{\textbf{RQ1:}} How do different strategies of data quality control affect the performance of synthetic data, and what strategy works the best? \underline{\textbf{RQ2:}} Which data synthesis strategy performs optimally for improving student model math reasoning? \underline{\textbf{RQ3:}} With a fixed compute for synthetic problem generation, should we mix data from multiple strategies or just scale the best strategy? \underline{\textbf{RQ4:}} How does the choice of problem generation and solution generation models impact performance with math synthetic data?


To address this lack of a unified experimental setup, and to optimize student model performance gains on math reasoning, we propose the \underline{F}ramework for \underline{L}LM \underline{A}ssessment of \underline{M}ath r\underline{E}asoning with Data \underline{S}ynthesis (FLAMES). Figure \ref{fig:overview} shows the flow diagram for the FLAMES framework. Based on extensive controlled experiments covering various aspects of the math reasoning data synthesis pipeline, we create a comprehensive list of design decisions and choose fixed values for each within the FLAMES framework. The FLAMES framework allows us to compare ten existing data synthesis strategies for improving student model performance across five benchmark math reasoning datasets. % accounting for various factors such as dataset scale,   As part of this framework, we create a comprehensive list of the setup choices that may impact performance within the math synthetic data pipeline, and we choose fixed values for them based on existing literature and our experimental findings. %FLAMES is a generic framework and can be easily extended with new setup choices.

Our controlled experiments and the FLAMES framework provide valuable insight into math reasoning data synthesis. \underline{\textbf{First}}, we find that data agents designed to increase problem complexity lead to best improvements on most math metrics. \underline{\textbf{Second}}, with a fixed data generation budget, keeping higher coverage of problems (even with some inaccuracy) is more important than keeping only problems with reliable solutions. \underline{\textbf{Third}}, synthetic data generated based on GSM8K and MATH can lead to improvements on competition-level benchmarks, showcasing easy-to-hard generalization capability with synthetic math data. \underline{\textbf{Fourth}}, choice of solution generation model plays a much bigger role than choice of problem generation model.

% should this paragraph be longer?
Using these and other findings from the FLAMES framework, we identify two areas of weakness in existing data synthesis strategies. First, existing strategies struggle to improve out-of-domain LLM math reasoning, beyond GSM8K \cite{cobbe2021training} and MATH \cite{hendrycks2measuring}. Second, as shown in prior work \cite{li2024gsm}, we find that existing strategies struggle to improve robustness to distracting information contained in math problems. We design two novel math data agents to target these weaknesses, showing improvement on relevant benchmarks compared to existing agents. 

% moving so its at the top of its page
%\vspace*{-7cm}
\begin{figure*}[t]
 \centering
  \includegraphics[width=1.8\columnwidth]{figures/overview_draftv3.png}
  \caption{The FLAMES Framework. By fixing each process in the data synthesis pipeline based on controlled experiments and prior work, the FLAMES framework enables evaluation of synthetic data agents in a unified environment. Processes for which we run \textbf{controlled experiments} are in bold font.}
  \label{fig:overview}
\end{figure*}
%\vspace*{-7cm}

Prior approaches to developing synthetic math reasoning datasets primarily utilize a single data synthesis strategy \cite{scalequest, omi2}. Using findings from the FLAMES framework about strengths and weaknesses of the 10 existing and 2 novel data synthesis strategies, we develop a SOTA blend of synthetic math reasoning data for LLM fine-tuning. We call this the FLAMES dataset, and we show that using this dataset at various scales (150K-1.5M) improves LLM math reasoning beyond existing math reasoning datasets (see Figure \ref{fig:experiments}).

% Using the FLAMES framework, we then design two novel agents targeting out-of-domain (OOD) generalization and robustness to adversarial problems. We demonstrate that data generated with these two agents lead to big performance gains on CollegeMath (evaluating out-of-domain) and GSMPlus (evaluating robustness), respectively. We use our FLAMES framework to perform a systematic comparison of 10 existing data agents from literature and our 2 novel data agents and provide key findings. We hope that this framework serves as a reference point for design and comparison of future math synthetic data research.

% Rewriting for flow/clarity
% To address this lack of a standard experimental setup, we propose a \underline{F}ramework for \underline{L}LM \underline{A}ssessment of \underline{M}ath r\underline{E}asoning with Data \underline{S}ynthesis (FLAMES). Figure \ref{fig:overview} shows the flow diagram for the FLAMES framework. As part of this framework, we create a comprehensive list of the setup choices that may impact performance within the math synthetic data pipeline, and we choose fixed values for them based on existing literature and our experimental findings. %FLAMES is a generic framework and can be easily extended with new setup choices.
%The Agentic FOX framework treats synthesis strategies as \textit{agents} which interact with teacher models and seed knowledge to synthesize novel math reasoning problems. Solutions to these problems are then synthesized in a unified manner, and a fixed amount of synthesized data is used to perform supervised fine-tuning (SFT) for a student model. By evaluating the fine-tuned student models on relevant math reasoning benchmarks, we can directly compare the performance of various math reasoning data synthesis strategies. %The Agentic FOX framework is designed based on extensive experiments and prior work, fixing the solution synthesis model, quality control measures, dataset size, underlying student model, fine-tuning parameters, and evaluation protocols. This framework is designed to enable swift evaluation of future data synthesis methods. 

% Rewriting for flow/clarity
% Additionally, we design two novel agents targeting out-of-domain (OOD) generalization and robustness to adversarial problems, and demonstrate with the FLAMES framework that data generated with these two agents lead to big performance gains on CollegeMath (evaluating out-of-domain) and GSMPlus (evaluating robustness), respectively. We use our FLAMES framework to perform a systematic comparison of 10 existing data agents from literature and our 2 novel data agents and provide key findings. We hope that this framework serves as a reference point for design and comparison of future math synthetic data research.

% Moving the research questions to before the framework intro for clarity (feel free to revert)
% We utilize the FLAMES framework to study several previously-under-studied research questions about math reasoning data synthesis. \underline{\textbf{RQ1:}} How do different strategies of data quality control (e.g. removing unsolvable problems) affect the performance of synthetic data, and what strategy works the best? \underline{\textbf{RQ2:}} Which data synthesis strategy performs optimally? \underline{\textbf{RQ3:}} With a fixed compute for synthetic problems generation, should we mix data from multiple strategies or just scale the best strategy? \underline{\textbf{RQ4:}} How does the choice of problem generation and solution generation models impact performance with math synthetic data? 

% Moving/editing for clarity
%Our work provides multiple valuable insights for synthetic data generation. \underline{First}, we find that data agents designed to increase problem complexity lead to best improvements on most math metrics. \underline{Second}, with a fixed data generation budget, keeping higher coverage of problems (even with some inaccuracy) is more important than keeping only problems with reliable solutions. \underline{Third}, synthetic data generated based on GSM8K and MATH can lead to improvements on competition-level benchmarks, showcasing easy-to-hard generalization capability with synthetic math data. \underline{Fourth}, choice of the solution generation model plays much bigger role than the choice of the problem generation model.

% Preserving previous version
% We utilize Agentic FOX framework to answer several previously-under-studied research questions about synthetic math reasoning data synthesis. \textbf{RQ1:} Role of Which synthetic data quality control strategy leads to most positively impact performance of underlying student models? \textbf{RQ2:} Which math data synthesis strategy leads to best improve in-domain, out-of-domain, robustness, and competition-level reasoning of underlying student models? \textbf{RQ3:} Which teacher models are best suited for problem and solution generation?the FLAMES dataset, which is the first math synthetic dataset that relies completely on permissively-licensed, open source models and does not use any proprietary model\footnote{ScaleQuest uses GPT-4o for preference optimization, and OpenMathInstruct-2 uses Llama3.1-405B-Instruct, which has a commercially restricted license.}. The FLAMES dataset consists of problems from four agents, and is designed to achieve optimal performance across in-domain, out-of-domain, robustness and competition-level metrics. Our experiments with DeepSeek-7B-base as the student model establish that our FLAMES dataset leads to drastic improvements with gains (in points) of +15.7 for OlympiadBench, +4.5 for CollegeMath, +6.5 for GSMplus and +3.1 for Math over the best public synthetic datasets. Further, as seen in Figure \ref{fig:experiments}, fine-tuning Qwen2.5-Math-Base with only our FLAMES dataset leads to Math score of 81.4, surpassing much larger open-source models (such as Llama3 405B) and proprietary models (such as GPT-4o and Claude 3.5 Sonnet).



In summary, our paper has the following contributions.

\begin{enumerate}
    \item We propose the FLAMES framework for controlled comparison of existing and future math problem synthesis strategies. We leverage this framework to compare ten existing data synthesis strategies across five evaluation datasets. 
    \item We design two novel data synthesis agents and empirically establish that they lead to enhanced robustness and out-of-domain improvements compared to existing data agents.
    \item We perform a rigorous study of multiple factors that impact performance with synthetic data pipeline. We provide valuable insights for researchers and practitioners working on improving LLM reasoning with synthetic data.  
%    \item We perform a rigorous study of multiple important axes of math reasoning data synthesis, including 1) synthetic problem and solution quality control methods, 2) problem generation agents, 3) problem generation models, and 4) solution generation models. This study yields several major findings.
    \item We develop three FLAMES datasets, which utilize only open source models and show drastic improvements over existing public math datasets.
\end{enumerate}

% Adding this to wrap the intro
We hope that our experimental findings, the FLAMES framework, our two novel data synthesis strategies, and the FLAMES datasets serve as a reference point for design and comparison of future research in math reasoning data synthesis.



% Preserving previous version for easy access
%Solving math problems has been a key measure of evaluating the reasoning ability of large language models (LLMs) in the field of natural language processing (NLP) \cite{wei2022chain, cobbe2021training, hendrycks2measuring}. Due to the challenges of creating a large-scale human-crafted dataset, various data synthesis strategies have been explored and proven effective in improving LLM math reasoning capabilities \cite{metamath, kpdds, scalequest}. Early works focused on synthesizing novel solutions to existing problems, which can be verified using ground truth solutions \cite{omi1, yuan2023scaling}. Recent works shifted focus towards increasing problem diversity by synthesizing novel math word problems and corresponding solutions \cite{kpdds, omi2, metamath}. \ignore{The common goal of proposed math problem synthesis strategies is to use one or more performant teacher models to synthesize pairs of math problems and solutions, which are used to improve the math reasoning ability of underlying student models via post-training. }This strategy has been shown to greatly improve LLM reasoning capabilities, with recent work showing that fine-tuning with only synthetic math reasoning data can create successful math specialist models with state-of-the-art (SOTA) performance on relevant benchmarks \cite{scalequest}. %\textcolor{blue}{(FIXME maybe a sentence or two here about how these works have shown to greatly improve reasoning of underlying student models via SFT and DPO, using percentages. We could also talk about how this has been used to create successful math specialist models, which are the SOTA on relevant benchmarks).} %Some works pose the math word problem synthesis task as data augmentation, using existing human-written problems to seed the synthesis of novel problems \cite{}. Other works synthesize problems using only a math specialist teacher model. 

% While a great deal of work has gone into developing various math reasoning data synthesis methods, prior works operate in isolated evaluation environments. Various works use different teacher models (including closed-source teacher models at different points in time), student models, quality control methods, amounts of synthesized data, training hyperparameters, and evaluation protocols. This landscape renders comparison of proposed synthesis strategies impractical, leaving researchers guessing as to what really drives the performance improvement.


%Further, the lack of standardization in prior work means little is known about the comparative impact of data quality control methods for math reasoning data synthesis, such as LLM-based filtering (e.g. removing unsolvable problems) \cite{scalequest} or solution consistency filtering \cite{prasad2024self}.

% replaced the last sentence here.
% Further, the ScaleQuest paper claims that using a 7B open source model to generate math problems from scratch provides more gains than existing open-source datasets. However, we argue that the reported gains could be due to use of a stronger problem synthesis model, as we establish in Section \ref{sec:data-agents-exp} that Suggester-Editor leads to better performance gains than QFT.

%As these strategies are generic and can be used with any LLM for problem synthesis, we term these strategies as data agents.

==> sections/02_RelatedWorks.tex <==
\section{Related Works}

\subsection{LLM Math Reasoning}

% Question -- would it be appropriate here to cite amazon nova? I will cite other recent LLMs to point out that math reasoning is an important metric.
The ability to solve math word problems is considered a key measure of large language model performance \cite{cobbe2021training, hendrycks2measuring}. Recent large language models have used math reasoning as an important metric to highlight model reasoning capability \cite{hendrycksmeasuring, team2024gemma, dubey2024llama, yang2024qwen2, deepseekai2025deepseekr1incentivizingreasoningcapability}. Various strategies have been proposed to improve large language model performance on math reasoning, including instruction tuning \cite{luo2023wizardmath, scalequest}, prompting techniques \cite{wei2022chain, chia2023contrastivechainofthoughtprompting}, and solution construction \cite{omi1}. Our work focuses on evaluating problem synthesis techniques for improving LLM math reasoning \cite{kim2024evaluatinglanguagemodelssynthetic, hase2024unreasonableeffectivenesseasytraining, he2024guidingcomplexitymakesgood}. 

\subsection{Data Synthesis for LLM Math Reasoning}

Existing works in evaluating synthetic data agents for improving LLM math reasoning have shown that various methods for generating synthetic math word problems can improve downstream performance of underlying student models fine-tuned on synthetic problems \cite{chen2025advancingmathreasoninglanguage}. MetaMathQA \cite{metamath} rewrites questions from multiple perspectives, enabling augmentation without additional knowledge. Open-Math-Instruct-2 uses few-shot LLM prompting to generate novel problems \cite{omi2}. Other works introduce multi-step approaches to synthesizing questions \cite{orcamath, luo2023wizardmath, mmiqc}.

==> sections/04_Agents.tex <==
\section{Data Synthesis Agents}
\label{sec:data-agents}
We select $10$ existing problem generation agents based on recent works in math reasoning data synthesis (refer Appendix . Based on the primary objective of these agents, we categorize them as one of the four categories: 1) In-domain practice, 2) In-domain complexity enhancing, 3) Robustness enhancing, and 4) Out-of-domain enhancing. %This categorization helps with designing new data agents, specifically addressing a category. 
Additionally, based on experimental findings detailed in Section \ref{sec:data-agents-exp}, we propose two novel agents under the categories of robustness enhancement and out-of-domain enhancement. We describe these 12 agents here. Prompts for each agent are provided in Appendix \ref{app:agent-prompts}.

\subsection{Existing Agents}
% \subsection{In-Domain Practice} 
\textbf{In-Domain Practice:} In-domain practice agents are designed to increase the amount of in-domain data available for model training. The goal of in-domain practice agents is to synthesize a large amount of math word problems which are similar in complexity, topic, and grade-level to problems in the training data. The \textbf{Few-Shot} agent, proposed in \cite{omi2}, uses existing problems as in-context examples to generate a novel problem. The \textbf{Paraphrasing} agent (\cite{metamath}) paraphrases existing problems. \cite{kpdds} introduce the use of key concepts as an intermediate problem representation for synthesizing novel problems. We evaluate a \textbf{Key Concepts} agent, which first extracts key concepts from an existing problem, and then uses those key concepts to generate novel problems. The related \textbf{Seeded Key Concepts} agent uses both extracted key concepts and the original existing problem to guide the generation of novel problems.

% \subsection{In-Domain Complexity Enhancing}
\textbf{In-Domain Complexity Enhancing:} There have been several proposed agents which aim to increase the complexity of existing math word problems \cite{orcamath, mmiqc, luo2023wizardmath}. The \textbf{Suggester/Editor} agent first suggests edits for problems to introduce additional reasoning steps, then synthesizes a novel problem by making those edits \cite{orcamath}. The \textbf{Iterative Question Composing (IQC)} agent turns an existing problem into a subproblem of a more complex synthetic problem \cite{mmiqc}. Both the Suggester/Editor and IQC agents may repeat their processes multiple times.

% \subsection{Robustness Enhancing}
\textbf{Robustness Enhancing:} Some proposed agents aim to alter existing problems to increase the robustness of the student model's reasoning process. These agents include the \textbf{Ask Me Anything} agent \cite{orcamath}, which converts an existing problem and solution into a statement, then prompts the teacher model to ask questions about the statement. Similarly, the \textbf{Self-Verification} agent \cite{metamath} converts an existing problem and solution into a statement, then replaces a number in the problem with a variable and asks the model to reason backwards to obtain the value of the variable. The \textbf{FOBAR} agent \cite{metamath} is similar to Self-Verification, except instead of having the teacher model rewrite the problem and solution into a statement before variable replacement, there is a template sentence added to the end of the problem which includes the problem's answer and the resulting question\footnote{See Appendix \ref{app:agent-prompts} for specific prompts}.

% \subsection{Out-of-Domain Enhancing} 
\textbf{Out-of-Domain Enhancing:} Recently, \cite{scalequest} proposed a method for synthesizing math reasoning data by using only a ``small-size'' (e.g. 7B) open-source model without a complex augmentation strategy. Their method revolves around the \textbf{Question Fine-Tuning (QFT)} process, which lightly fine-tunes a 7B math specialist model on the GSM8K and MATH training datasets, then prompts the fine-tuned model with only the system prompt to synthesize novel math word problems. We replicate their proposed process using Qwen2.5-Math-7B-Instruct \cite{yang2024qwen2} to create the QFT agent, designed to enhance general math reasoning performance. We call this an out-of-domain agent, as the agent prompt is not seeded with any specific in-domain problem.

\subsection{Novel Agents}

\begin{figure}[t]
 \centering
  \includegraphics[width=\columnwidth]{figures/novel_agentsv2.png}
  \caption{Illustrating examples of our novel Distraction Insertion and Taxonomy-Based Key Concepts data synthesis agents.}
  \label{fig:agents}
\end{figure}

% \textcolor{blue}{FIXME maybe we can include a figure here where we show how these two novel agents work... So we can get a sense of what the agents look like generally too}

%In addition to the 10 previously-proposed agents which we evaluate in the Agentic FOX framework, we introduce 2 novel agents aimed at increasing the out-of-domain performance and robustness of the student model. 
We propose \textbf{Taxonomy-Based Key Concepts} and \textbf{Distraction Insertion} as two novel agents. See Figure \ref{fig:agents} for examples of problem generation with these agents. The \textbf{Taxonomy-Based Key Concepts} agent uses a curated taxonomy of math subjects to generate key concepts needed to understand those subjects, and then uses each key concept to synthesize novel problems for them. This agent is not seeded with in-domain GSM8K or MATH training problems, rather it is seeded with taxonomy subjects from a variety of sources \cite{kpdds, liu2024mathbenchevaluatingtheoryapplication, huang2024mustardmasteringuniformsynthesis, didolkar2024metacognitivecapabilitiesllmsexploration},  and it is considered an out-of-domain enhancing agent. 

\cite{li2024gsm} have shown that LLMs are susceptible to reason poorly when adversarial, distracting information is added to existing math word problems. With the goal of increasing reasoning performance in the presence of such distracting information, we introduce the \textbf{Distraction Insertion} agent, a robustness-enhancing agent which is designed to insert distracting information into existing seed problems.

==> sections/06_Dataset.tex <==

% \section{FLAMES Dataset}

%Several works introduce synthetic training datasets for math reasoning of different sizes. The OrcaMath dataset utilizes the Ask Me Anything and Suggester/Editor strategies to synthesize 200k training pairs \cite{orcamath}. The MMIQC dataset contains 1.2m training pairs generated using the IQC agent, with 221k being unique synthetic problems \cite{mmiqc}. The MetaMathQA dataset comprises 395k training pairs, of which 146k are unique, synthesized using paraphrasing, FOBAR, and self-verification agents \cite{metamath}. OpenMathInstruct-2 consists of 14m training pairs, including 600k unique problems created via few-shot prompting \cite{omi2}. The ScaleQuest dataset features 1m unique problems generated with the QFT agent \cite{scalequest}. 

% We use the findings of the Agentic FOX framework, with the goal of isolating data synthesis strategies from their unique evaluation environments, enable us to develop a SOTA large-scale synthetic math reasoning dataset, which we compare against these existing datasets. 

% We leverage our findings from the FLAMES framework, including our systematic study of the 12 data agents and other factors impacting synthetic data, to construct the FLAMES dataset. This dataset is a mixture of superior data synthesis agents across all four agent types (refer Section \ref{sec:data-agents}), designed to provide balanced performance across multiple benchmarks. We experiment with multiple mixing proportions (refer to experiments in Appendix \ref{app:combining-agents}) and found the best results by mixing 50\% Suggester-Editor, 20\% IQC, 20\% Taxonomy Key Concept (our proposed) and 10\% Distraction Insertion (our proposed) agents. We develop 3 versions of the FLAMES dataset - FLAMES\_small (150K), FLAMES\_large (1M), and FLAMES\_xl (1.45M). We use FLAMES\_small for comparison with individual agents (Section \ref{sec:data-agents-exp}), and FLAMES\_large (1M) and FLAMES\_xl (1.5M) for comparison with existing math datasets such as NuminaMath and ScaleQuest (Section \ref{sec:os-dataset-exp}).

%We call this dataset the FOXMath Large dataset. Detailed in Section \ref{sec:os-dataset-exp}, our extensive experiments using 5 different underlying student models shows that FOXMath Large outperforms the previous SOTA synthetic math dataset across 5 benchmark datasets.


%a combination of all four agent types to construct a dataset which has balanced performance across all 4 dimensions. We study different mixing synthetic data with different proportions and found best results with XX. We develop 3 versions of Math data with synthetic problems and solutions - openmathsynthetic_xl (1.45M), openmathsynthetic_large (1M) and openmathsynthetic_small (150K).


%We aim to use the findings of the Agentic FOX framework to produce a dataset which approximates an optimal blend of synthesized data in terms of student model downstream performance on the benchmarks in Section \ref{sec:eval-benchmarks}. We do this by finding and scaling a ratio of data from several performant data synthesis agents introduced in Section \ref{sec:data-agents}. Our large-scale synthetic dataset is 1 million pairs of synthetic math word problems and solutions. 50\% of this dataset is sourced from the Suggester/Editor agent, 20\%  from the IQC agent, 20\% from the novel Taxonomy Key Concepts agent, and 10\% from the novel Distraction Insertion agent. We call this dataset the FOXMath Large dataset. Detailed in Section \ref{sec:os-dataset-exp}, our extensive experiments using 5 different underlying student models shows that FOXMath Large outperforms the previous SOTA synthetic math dataset across 5 benchmark datasets.

% Several works introduce synthetic training datasets for math reasoning of different sizes. The OrcaMath dataset utilizes the Ask Me Anything and Suggester/Editor strategies to synthesize 200k training pairs \cite{orcamath}. The MMIQC dataset contains 1.2m training pairs generated using the IQC agent, with 221k being unique synthetic problems \cite{mmiqc}. 

% MetaMathQA 395k total 146k unique via paraphrasing, FOBAR, self-verification agents
% OpenMathInstruct-2 is 14M total with 600k unique via few-shot
% ScaleQuest is 1M total unique with QFT agent

==> tables/ProbSol_Models.tex <==
\begin{table*}[ht]
    \centering
    \setlength\tabcolsep{4pt} % Reduce horizontal padding
    \resizebox{\textwidth}{!}{ % Resize table to fit within page width
    \begin{tabular}{|c|c|c|c|c|c|c|} \hline
        Problem Generation Model &Solution Generation Model &Underlying Model &GSM8K &MATH5K &Average \\ \hline
        & &DeepSeek-Math-7B (Reported) &64.2 &36.2 &50.2 \\ \hline
        Qwen2.5-32B-Instruct &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &82.5 &56.4 &69.5 \\
        DeepSeek-v2.5 &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &83.5 &54.9 &69.2 \\
        Mix &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &83.5 &56.0 &69.8 \\ \hline
        Qwen2.5-32B-Instruct &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &82.5 &56.4 &69.5 \\
        Qwen2.5-32B-Instruct &DeepSeek-Math-7B-RL &DeepSeek-Math-7B &85.1 &49.3 &67.2 \\
        Qwen2.5-32B-Instruct &Mix &DeepSeek-Math-7B &84.5 &51.4 &68.0 \\ \hline
        \end{tabular}
    }
    \caption{Impact of varying problem and solution generation models on underlying student model performance.}
    \label{tab:probsolmodels}
\end{table*}

==> tables/ProbSol_Modelsv2.tex <==
\begin{table*}[ht]
    \centering
    \setlength\tabcolsep{4pt} % Reduce horizontal padding
    \resizebox{\textwidth}{!}{ % Resize table to fit within page width
    \begin{tabular}{|c|c|c|c|c|c|c|} \hline
        Problem Generation Model &Solution Generation Model &Underlying Model &GSM8K &MATH5K &Average \\ \hline
        & &DeepSeek-Math-7B (Reported) &64.2 &36.2 &50.2 \\ \hline
        Qwen2.5-32B-Instruct &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &82.5 &56.4 &69.5 \\
        DeepSeek-v2.5 &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &83.5 &54.9 &69.2 \\
        % Mix &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &83.5 &56.0 &69.8 \\ \hline
        % Qwen2.5-32B-Instruct &Qwen2.5-Math-7B-Instruct &DeepSeek-Math-7B &82.5 &56.4 &69.5 \\
        Qwen2.5-32B-Instruct &DeepSeek-Math-7B-RL &DeepSeek-Math-7B &85.1 &49.3 &67.2 \\\hline
        % Qwen2.5-32B-Instruct &Mix &DeepSeek-Math-7B &84.5 &51.4 &68.0 
        \end{tabular}
    }
    \caption{Impact of varying problem and solution generation models on underlying student model performance.}
    \label{tab:probsolmodels}
\end{table*}

==> tables/Quality_Control.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
\textbf{Method} &\textbf{Dataset Size} &\textbf{Precision} &\textbf{Coverage} &\textbf{GSM8K} &\textbf{MATH5K} &\textbf{Average} \\ \hline
\multicolumn{7}{|c|}{\textbf{Coverage-Dependent}} \\ \hline
Self-Consistency &45K &Very High &0.30 &82.90 &56.40 &69.65 \\
Majority &90K &High &0.60 &84.50 &59.40 &71.95 \\
Solvability + RM &70K &High &0.47 &84.50 &57.90 &71.20 \\
Majority + First &150K &Medium &1.00 &\underline{86.40} &60.90 &\underline{73.65} \\
Solvability + First &70K &Low &0.47 &84.10 &58.20 &71.15 \\
First &150K &Low &1.00 &84.80 &\underline{61.10} &72.95 \\ \hline
\multicolumn{7}{|c|}{\textbf{Coverage-Independent}} \\ \hline
Self-Consistency &45K &Very High &- &82.90 &56.40 &69.65 \\
Majority &45K &High &- &82.00 &56.10 &69.05 \\
Solvability + RM &45K &High &- &82.90 &56.30 &69.60 \\
Majority + First &45K &Medium &- &83.00 &\underline{56.60} &\underline{69.80} \\
Solvability + First &45K &Low &- &83.20 &55.60 &69.40 \\
First &45K &Low &- &\underline{83.40} &55.80 &69.60 \\ \hline
\end{tabular}
\caption{Coverage-Dependent and Coverage-Independent results for various synthetic data quality control strategies.}
\label{tab:quality-control}
\end{table*}

